MAtch, eXpand and Improve: Unsupervised Finetuning for Zero-Shot Action Recognition with Language Knowledge

Large scale Vision-Language (VL) models have shown tremendous success in aligning representations between visual and text modalities. This enables remarkable progress in zero-shot recognition, image generation & editing, and many other exciting tasks. However, VL models tend to over-represent objects while paying much less attention to verbs, and require additional tuning on video data for best zero-shot action recognition performance. While previous work relied on large-scale, fully-annotated data, in this work we propose an unsupervised approach. We adapt a VL model for zero-shot and few-shot action recognition using a collection of unlabeled videos and an unpaired action dictionary. Based on that, we leverage Large Language Models and VL models to build a text bag for each unlabeled video via matching, text expansion and captioning. We use those bags in a Multiple Instance Learning setup to adapt an image-text backbone to video data. Although finetuned on unlabeled video data, our resulting models demonstrate high transferability to numerous unseen zero-shot downstream tasks, improving the base VL model performance by up to 14\%, and even comparing favorably to fully-supervised baselines in both zero-shot and few-shot video recognition transfer. The code will be released later at \url{https://github.com/wlin-at/MAXI}.

==> tex/abstract_leonid.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
% \wei{For co-authors: Careful, abstrac and introduction (current version is from some time ago) needs to be re-written to be coherent with the method section. Method section is already pretty complete. }
    Large scale \vlfull{} (\vl{}) models have shown fantastic results in terms of aligning between visual and text modalities representations enabling great progress in \zsfull{} recognition, image generation \& editing, and many other exciting tasks. However, these models still have some fundamental weaknesses requiring additional training before applying them to \zsfull{} action recognition tasks. For example, \vl{} models tend to over-represent objects while paying much less attention to verbs, and require additional tuning on video data for best \zsfull{} action recognition performance.
    While previous work relied on large (expensive to obtain) supervised data, in this work we propose an unsupervised approach. We adapt a \vl{} model for zero-shot and few-shot action recognition using a collection of unlabeled videos and a set of language sources, such as unpaired action dictionaries, Large Language Models, and \vl{} models for matching and captioning. 
    % We attain improvement of up to XXX\% in \zs{} transfer to novel action recognition tasks, in some cases even improving upon supervised baselines by up to YYY\%.
    Although finetuned on unlabeled video data, our resulting models demonstrate high transferability to numerous unseen zero-shot downstream tasks, improving the base \vl{} model performance by up to 14\%, and even comparing favorably to fully-supervised baselines in both zero-shot and few-shot video recognition transfer.
    The code is provided in supplementary and will be released upon acceptance.
    
   % The ABSTRACT is to be in fully-justified italicized text, at the top
   % of the left-hand column, below the author and affiliation
   % information. Use the word ``Abstract'' as the title, in 12-point
   % Times, boldface type, centered relative to the column, initially
   % capitalized. The abstract is to be in 10-point, single-spaced type.
   % Leave two blank lines after the Abstract, then begin the main text.
   % Look at previous ICCV abstracts to get a feel for style and length.
\end{abstract}

==> tex/intro_leonid_new.tex <==
\section{Introduction}
% \wei{For co-authors: Careful, introduction needs to be re-written to be coherent with the method section. Method section is already pretty complete. }
% \wei{Some bullet points for the introduction flow: \\
% - People have done Vl adaptation for video, but only with fully supervised data (annotated clips\\
% - People have done VL finetuning from unpaired data\\
% - we proposed to combine those two ideas and propose the first approach that does finetune a VL model from unpaired videos and given class information without any connection between the two \\
% - the scenario in this case work as follows: During training, we're given a set of unlabeled videos as well as a target dictionary with possible labels for the video set\\
% - and then describe method ... text bag to augment class labels and improve unpaired data matching\\
% }

 \vlfull{} (\vl{}) models \cite{clip, blip, jia2021scaling} have met unprecedented success in terms of unlocking many vision applications \cite{clip} to work with potentially unlimited output vocabularies through the promise of \zsfull{} transfer \cite{zhang2021tip,zhou2022conditional,zhou2022learning,gu2021open,rasheed2022bridging,zhou2022detecting,li2022language,rao2022denseclip} enabled by the alignment between visual and language (text) representation spaces effectively attained by those models leveraging huge amounts of paired image and text data. Incorporating a \vl{} model as a source (base) model or as an architectural component has allowed scaling fine-tuning on relatively small, compared to the vast \vl{} pretraining, datasets (e.g. limited in terms of the number of observed objects or other visual concepts) towards \zsfull{} transfer at inference time. That is recognizing \cite{zhang2021tip,zhou2022conditional,zhou2022learning}, detecting \cite{gu2021open,rasheed2022bridging,zhou2022detecting}, segmenting \cite{li2022language,rao2022denseclip}, and even generating \cite{dreambooth} objects unseen during the finetuning stage and only encountered for the first time during the inference. 

 % However, despite all this progress, when applied directly to video data \vl{} models have been observed to suffer from several shortcomings \cite{a,b,c}. Being trained on enormous image + text paired datasets commonly makes them somewhat more vulnerable to video artifacts such as video compression and motion blur. More importantly, as has been extensively studied in several works \cite{winoground,vl-checklist,aro-benchamrk} the \vl{} models have a tendency to mostly represent the objects (nouns) appearing on the images (or video frames) resulting in a kind of `bag of object' representation while paying much less attention to visual details that would correspond to attributes (adjectives) or actions (verbs) in the language counterpart. Intuitively, both of these factors negatively affect direct \vl{} model applications to \zsfull{} action recognition resulting in significant performance drops compared to common image-based more `object-oriented' tasks. 

However, despite all this progress in \zsfull{} image tasks, \vl{} models have been observed to underperform  when applied to \zsfull{} action recognition video data without any finetuning \cite{wang2021actionclip,ni2022expanding,ju2022prompting,wu2023revisiting,castro2022fitclip,rasheed2022fine}. 
% Being trained on enormous image + text paired datasets commonly makes them somewhat more vulnerable to video artifacts such as video compression and motion blur. More importantly, 
A possible reason for this might be that,
as has been extensively studied in several works \cite{winoground,vlc,aro}, the \vl{} models have a tendency to mostly represent objects (nouns) and not actions (verbs or verb phrases).
%
Therefore, to deal with these shortcomings of \vl{} models w.r.t. \zsfull{} action recognition, previous works \cite{wang2021actionclip,ni2022expanding,ju2022prompting,wu2023revisiting,castro2022fitclip,rasheed2022fine} have used (expensive to obtain) supervised datasets (e.g. K400 \cite{kay2017kinetics}) for fine-tuning of \vl{} models (e.g. the most popular CLIP \cite{clip}) towards improved video \zsfull{} recognition performance. The potential downsides of this approach are: (i) reliance on large-scale supervised action datasets that are expensive to collect; (ii) the exposure of the model to only the limited action vocabulary during the supervised fine-tuning (e.g. 400 actions of K400 vs. over 8K possible single verb actions and much more possible general actions in English language) limiting the performance of \zsfull{} transfer to unseen action categories. 
% So the questions we ask in this work are: (i) is it possible to tune strong large-scale pre-trained \vl{} models towards effective \zs{} transfer for action recognition while only leveraging unlabeled video data? (ii) is it possible to harness the knowledge of language to go beyond the limited action vocabulary available for action datasets?

 % In our work, we answer both questions in the affirmative. 
We propose `\oursfull{}' (\OurMethod) -- the first approach to allow finetuning on completely unlabeled video data (e.g. unlabeled K400 \cite{kay2017kinetics}) and a set of language sources, such as unpaired action dictionaries, Large Language Models (e.g. GPT \cite{brown2020language}), and \vl{} models for matching (e.g. CLIP \cite{clip}) and captioning (e.g. BLIP \cite{blip}). As illustrated on Figure \ref{fig:teaser}, \OurMethod effectively leverages the different language sources for collecting and refining noisy bags of potential text that may correspond to each video in the unlabeled set and then applies Multiple Instance Learning (MIL) for finetuning the \vl{} model using those bags.
We extensively evaluate \OurMethod on 7 downstream \zsfull{} and few-shot transfer action recognition benchmarks completely unseen during training. We show that \OurMethod is effective in leveraging unlabeled video data, not only significantly (up to 14\%) improving the source \vl{} model performance on all of those tasks, but also favorably competing with state-of-the-art supervised methods trained on fully supervised counterparts of the same finetuning data, and even improving upon them in some zero-shot and few-shot action recognition transfer tasks.
% \zsfull{} and few-shot transfer action recognition performance to video benchmarks unseen during training. 
%
% Moreover, we show that to achieve this, we can effectively fuse unlabeled video data with `bags' of language knowledge mined from either vision-conditioned and/or pure language-conditioned sources. Specifically, for vision-conditioned, we match video representations to (large) action (language) vocabulary using CLIP \cite{clip} and/or produce a sequence of frame captions using BLIP \cite{blip}. For language-conditioned, we query an LLM (e.g. GPT 3.5 \cite{gpt3.5}) for possible expanded descriptions of texts obtained in vision-conditioned ways. Applying, Multiple Instance Learning (MIL) strategies (e.g. the recent MIL-NCE \cite{milNCE}) using these `language knowledge bags' as pseudo-labels for the unlabeled videos results in the aforementioned gains.

 To summarize, the contributions of this work are as follows: (i) we propose a new task of leveraging unlabled video collection and a set of language sources to improve downstream \zsfull{} and few-shot transfer action recognition performance for strong pre-trained \vl{} models; (ii) we propose \OurMethod{} -- a first approach for this task that effectively matches each video in the unlabeled collection with the corresponding `text bag' of language knowledge mined from the language sources and employs Multiple Instance Learning for finetuning a \vl{} model using these `text bags'; (iii) we extensively evaluate our approach on 7 action recognition benchmarks unseen during training and demonstrate up to 14\% absolute \zsfull{} performance improvements over the source \vl{} model, as well as significant improvements over baseline models trained on fully supervised versions of the same data; (iv) additionally, we show a significant (up to 2.8\%) improvements in the few-shot action recognition transfer scenarios compared to fully supervised baselines improving upon them in 10 out of 12 standard evaluations; and (v) we provide extensive ablations to validate our approach from multiple perspectives.

==> tex/introduction_leonid.tex <==
\section{Introduction\wei{For co-authors: Careful, introduction needs to be re-written to be coherent with the method section. Method section is already pretty complete. }}

\wei{Some bullet points for the introduction flow: \\
- People have done Vl adaptation for video, but only with fully supervised data (annotated clips\\
- People have done VL finetuning from unpaired data\\
- we proposed to combine those two ideas and propose the first approach that does finetune a VL model from unpaired videos and given class information without any connection between the two \\
- the scenario in this case work as follows: During training, we're given a set of unlabeled videos as well as a target dictionary with possible labels for the video set\\
- and then describe method ... text bag to augment class labels and improve unpaired data matching\\
}

 Large scale \vlfull{} (\vl{}) models \cite{clip, blip, ...,jia2021scaling} \wei{is ALIGN~\cite{jia2021scaling} large-scale VL?} have met unprecedented success in terms of unlocking many vision applications \cite{a,b,c} to work with potentially unlimited output vocabularies through the promise of \zsfull{} (\zs{}) transfer \cite{a,b,c,zhang2021tip,zhou2022conditional,zhou2022learning,gu2021open,rasheed2022bridging,zhou2022detecting,li2022language,rao2022denseclip} enabled by the alignment between visual and language (text) representation spaces effectively attained by those models leveraging huge amounts of paired image and text data. Incorporating a \vl{} model as a source (base) model or as an architectural component have allowed scaling fine-tuning on relatively small, compared to the vast \vl{} pretraining, datasets (e.g. limited in terms of the number of observed objects or other visual concepts) towards \zs{} transfer at inference time. That is recognizing \cite{a,b,c,zhang2021tip,zhou2022conditional,zhou2022learning}, detecting \cite{a,b,c,gu2021open,rasheed2022bridging,zhou2022detecting}, segmenting \cite{a,b,c,li2022language,rao2022denseclip}, and even generating \cite{dreambooth,others,like,it} objects unseen during the finetuning stage and only encountered for the first time during the inference. 

 However, despite all this progress, when applied directly to video data \vl{} models have been observed to suffer from several shortcomings \cite{a,b,c}. Being trained on enormous image + text paired datasets commonly makes them somewhat more vulnerable to video artifacts such as video compression and motion blur. More importantly, as has been extensively studied in several works \cite{winoground,vl-checklist,aro-benchamrk} the \vl{} models have a tendency to mostly represent the objects (nouns) appearing on the images (or video frames) resulting in a kind of `bag of object' representation while paying much less attention to visual details that would correspond to attributes (adjectives) or actions (verbs) in the language counterpart. Intuitively, both of these factors negatively affect direct \vl{} model applications to \zsfull{} action recognition resulting in significant performance drops compared to common image-based more `object-oriented' tasks. 

 Therefore, to deal with these shortcomings of \vl{} models w.r.t. \zs{} action recognition, previous works \cite{a,b,c} have proposed leveraging supervised fine-tuning of these models (e.g. the most popular CLIP \cite{clip}) on action datasets (e.g. K400 \cite{kinetics}) with the hopes that it would improve alignment to the video data on the visual representation side, while at the same time enhance the significance at least of a part of the (initially under-represented) action language vocabulary (verbs) in the \vl{} model's visual representation. The potential downsides of this approach are: (i) reliance on large-scale supervised action datasets that are expensive to collect; (ii) the exposure of the model to only the limited action vocabulary during the supervised fine-tuning (e.g. 400 actions of K400 vs. over 8K possible single verb actions and much more possible general actions in English language) limiting the performance of \zs{} transfer to unseen action categories. So the questions we ask in this work are: (i) is it possible to tune strong large-scale pre-trained \vl{} models towards effective \zs{} transfer for action recognition while only leveraging unlabeled video data? (ii) is it possible to harness the knowledge of language to go beyond the limited action vocabulary available for action datasets?

 In our work, we answer both questions in the affirmative. We show that unlabeled video data can be effectively used to significantly improve \zs{} transfer action recognition performance to unseen video benchmarks (e.g. unlabeled K400 \cite{k400} $\rightarrow$ HMDB \cite{hmdb}, UCF \cite{ucf}, and others). Moreover, we show that to achieve this, we can effectively fuse unlabeled video data with `bags' of language knowledge mined from either vision-conditioned and/or pure language-conditioned sources. Specifically, for vision-conditioned, we match video representations to (large) action (language) vocabulary using CLIP \cite{clip} and/or produce a sequence of frame captions using BLIP \cite{blip}. For language-conditioned, we query an LLM (e.g. GPT 3.5 \cite{gpt3.5}) for possible expanded descriptions of texts obtained in vision-conditioned ways. Applying, Multiple Instance Learning (MIL) strategies (e.g. the recent MIL-NCE \cite{milNCE}) using these `language knowledge bags' as pseudo-labels for the unlabeled videos results in the aforementioned gains.

 To summarize, the contributions of this work are as follows: (i) we propose a new task of leveraging unlabled video data to improve downstream \zs{} transfer action recognition performance for strong pre-trained \vl{} models; (ii) we propose a first method for approaching this task via effective fusing of the unlabeled data with the corresponding language knowledge mined via pre-trained large language and \vl{} models and employed through Multiple Instance Learning on the resulting corresponding text `bags'; (iii) we demonstrate significant relative improvements of up to XXX\% over strong baselines including the original pre-trained models and models tuned using large-scale supervised data, as well as show a significant (up to YYY\%) improvements in the few-shot tuning scenarios, also providing extensive ablations to validate our approach.

==> tex/method_mateusz.tex <==
\section{Method}
\mk{I know understand that I should have written `data set' where I wrote `batch';}
We adopt the classical approach to zero-shot classification with a vision-language model:
During inference, given a video $x$, a set of classes $\mathcal{C}$, and a text prompt $t_c$ for each $c\in \mathcal{C}$, we compute a prompt embedding using a text encoder $\phi_t$, and a video embedding using a video encoder $\phi_v$.
The zero-shot classification is performed by selecting the class $\hat c$ with the maximum similarity between its prompt and the video representation,
\begin{equation} \label{eq:classificationAtTestTime}
\hat c= \argmax_c \phi_v(x)^\top \phi_t(t_c).
\end{equation}
\mk{you do not need to normalize this }
% The zero-shot classification is performed by selecting the class prompt with the maximum similarity to the video representation, \ie, $\hat c= \argmax_c \bar \phi_v(x)^\top \bar \phi_t(t_c)$, 
% where $\bar \phi_v(x)$ and $\bar  \phi_t(t_c)$ denote the normalized video and text feature, respectively.

Like a number of existing methods~\cite{}, we build on top of CLIP.
We directly adapt CLIP's text encoder for $\phi_t$ and construct $\phi_v$ using CLIP's image encoder, as described in Sec.~\ref{sec:clip_on_video}.
Since CLIP is trained on 2D images, it does not capture video-specific cues, which compromises its performance in video recognition.
We remedy this by fine-tuning the model on a collection of unlabelled videos.
Our fine-tuning concept is based on a combination of pseud-labeling and Multiple Instance Learning: we align each video encoding $\phi_v(x)$ to \textit{text bags} --- possibly noisy collections of prompts --- representing other videos with the same pseudo label.
We describe our fine-tuning approach in Sec.~\ref{sec:mil-nce}.
The right composition of the text bags is essential for performance.
In Sec.~\ref{sec:text_bag_construction}, we propose to compose instance-specific, video-conditioned text bags by mixing prompts from different language sources.
An overview of our fine-tuning method is presented in Fig.~\ref{fig:pipeline}. 

\subsection{CLIP for Video Data}\label{sec:clip_on_video}

The network architectures employed by CLIP are designed for two-dimensional images.
To fully harness their power for video classification, we first need to adapt them to processing temporal frame sequences.
Previous efforts to extend CLIP to video data included adding modules dedicated to learning temporal relationships between frames~\cite{}.
However, it has been shown recently that simply pooling frame-level encodings makes the network implicitly model the temporal cues and outperforms more sophisticated architectures~\cite{rasheed2022fine,castro2022fitclip}.
We therefore follow this approach.
Given a video $x$, we pass its $M$ frames $(x[m])_{1\le m \le M}$ through the CLIP image encoder $\phi_\textrm{img}$ and compute the video representation
\begin{equation} \label{eq:videoEncoder}
\phi_{v}(x) = \sum_m \phi_\textrm{img}(x[{m}]) / M . 
\end{equation}
Since we introduce no additional parameters to the original CLIP encoder, pre-trained on a very large number of text-image pairs,
this delivers sufficient initial performance for fine-tunning with the approach we describe in Sec.~\ref{sec:mil-nce}. 
We also explored extending this architecture with a parameter-free temporal-aware module, but found out that it had negligible impact on performance.
The results can be found in the supplementary material.

\wei{as ViFiCLIP~\cite{rasheed2022fine} already outperforms related work with additional learnable components, maybe we do not have to explore this in supp anymore. need to discuss. }

\subsection{Fine-tuning the Network}\label{sec:mil-nce}

\mk{
I tried to write why you designed the loss like this, but it is not easy to see the intention behind this design. 
Have you tried aligning video encodings to encodings of the prompts corresponding to that same video? 
This is how Miech et al do it.
Also, I think Fig. 2 does not convey this video-to-video alignment
}

Fine tuning an \emph{image} vision-language model for \emph{video} classification is difficult, because 
some actions can be performed in different contexts, which makes their visual encoding align with different textual prompts, depending on the context.
For example, a photo of an archer at the Olympic Games is likely to be aligned with different text than a photo of a child handling a toy bow at a birthday party.
Moreover, the text space of a model trained on text-image pairs is biased towards objects as opposed to actions~\cite{}, but objects alone often provide insufficient cue for identification of certain actions.
To address these challenges, we employ a combination of pseudo-labeling with multiple instance learning.

\myparagraph{Pseudo-labeling.}
In a practical scneario, we usually have a coarse prior knowledge of the set of action classes $\mathcal{C}$ for an unannotated video collection.
For each action class $c\in\mathcal{C}$, we created the prompt $t_c$ using the names of the actions.
We compute the pseudo label for video $x_i$ as
\begin{equation}
\hat c_i= \argmax_{c\in D} {\phi_v(x_i)}^\mathsf{T}, \phi_t(t_c) .
\end{equation}
The pseudo-labels are noisy, especially at the beginning of the fine-tuning.
To reduce the influence of this noise on training, for each batch we only keep a fraction of $p$ videos with the highest cosine similarity to their matching prompt encoding.
As we will explain below, our use of the pseudo-labels is unorthodox: we do not enforce them on the network, but instead align representations of videos with the same pseudo-labels.

\myparagraph{Representing videos with text bags.}
We propose to represent each video $x_i$ in the batch with a \emph{text bag} --- a collection of diverse prompts, that represent both the pseudo label $\hat c_i$,
and the context in which the action appears in a given video.
Formally, the text bag for video $x_i$ is a set $T_i$ of prompts.
We detail the construction of $T_i$ in Sec.~\ref{sec:text_bag_construction}.
Each $t\in T_i$ is encoded by $\phi_t$, and we therefore obtain two representations of the unlabelled video $x_i$: its visual encoding $\phi_v(x_i)$ and the set of encodings of it text bag $\{\phi_t(t)\}_{t\in T_i}$.
The advantage of the text bag is that they represent many aspects of the video and the recorded action.
We will next argue that aligning text bags 
gives the network the liberty to represent different context of the same action with different visual encodings, while simultaneously requiring that the encoding is discriminative of the performed action.

\myparagraph{Aligning representations.}
We fine-tune the network by aligning the visual representation of each video to the text bag representations of all other videos with the same pseudo label in the batch.
In order to softly associate a bag of texts $T_i$ with each video $x_i$, in which one or multiple texts are a positive match to the video, 
we adapt the combination of Multiple Instance Learning and Noise Contrastive Estimation (MIL-NCE) by Miech et.\ al.~\cite{miech2020end}.
The loss function 
\begin{equation}
\small
    - \sum_{i} 
    \log 
    \frac{\sum_{j} \sum_{t\in T_j} \exp(\bar \phi_v(x_i)^\top \bar \phi_t (t)/\sigma)\cdot \mathbbm{1}(\hat c_i = \hat c_j)}
    {\sum_k\sum_{t\in T_k} \exp(\bar \phi_v(x_i)^\top \bar \phi_t (t)/\sigma)}
    % -l(i_j) \cdot \log (C^I(E(i_j; \theta^I_E) ; \theta^I_C ))
\end{equation}
where $i,j,k$ range over the batch elements, the bar denotes normalization to unit norm.
and $\sigma$ is a temperature parameter.
$\mathbbm{1}(\hat c_i = \hat c_j)$ is an indicator that $x_i$ and $x_j$ have the same pseudo-label.

\mk{note that you cannot really compute this loss if the summation is over the entire data set; Are you aware how it works? It could just be aligning each $\phi_v(x_i)$ to a single prompt.}

The advantage of this formulation is twofold.
First, it aligns representations softly, enabling aligning each video encoding to the encoding of one of many prompts attributed to other videos with the same pseudo-labels.
In other words, it lets the network preserve the diversity of its encodings, which is beneficial for zero-shot learning.
Second, since the text bags for different videos may be different even when their pseudo-labels are the same, it promotes alignment to prompts refering to concepts that may not appear in a given video, but are semantically related to the captured action.

\subsection{Text Bag Construction}\label{sec:text_bag_construction}
The composition of the text bags is essential to the performance of our fine-tuning technique. 
We initialize each text bag $T_i=\{ t_{\hat c_i}\}$, where $t_{\hat c_i}$ is the prompt obtained from the action name corresponding to the pseudo-label of $x_i$.
We then expand the text bags using GPT-3 and BLIP captioning.

\myparagraph{GPT-3 text expansion.} We expand the text bag by leveraging the large-scale language model (LLM) GPT-3~\cite{brown2020language}. This is similar to in-context learning \cite{} (\wei{is this correct?}) where few examples of desired output are provided in the context window of the input. By providing the best matched text $\hat t_i$ in the input prompt for LLM, we result in a collection of expanded alternative descriptions of the action. The descriptions contain hallucinating details leveraging the collective world knowledge of the LLM. 
We collect the verbs and verb phrases extracted from the generated expanded action descriptions. Furthermore, we perform text augmentation by including both the lemma and gerund (present participle) forms of the verbs. We add the collection of words to the text bag $T_i$. 
\wei{need to further check this paragraph}.

\myparagraph{BLIP captioning.} We employ the vision-language model BLIP~\cite{li2022blip} for generating captions of static frames on a video. Note that the image captioning model is not pretrained on any video domain. The frame captions provide instance-level descriptions that are dependent on the visual content of frames of the unlabeled videos. Similarly, we further collect verbs in the descriptions, and perform text augmentation. We include the collection of words to the text bag $T_i$. 



==> tex/supp_content.tex <==
For further insights into our approach \OurMethod, we provide source code (Sec.~\ref{sec:source_code}) in the supplementary. We introduce more dataset statistics (Sec.~\ref{sec:dataset_statistics}) and implementation details (Sec.~\ref{sec:implementation_detials}) of \OurMethod. 

In the additional results, we provide comparison of visualizations of attention heatmaps across several approaches in Sec.~\ref{sec:attention-heatmaps}. Furthermore, we report more results of finetuning with noisy action dictionary (Sec.~\ref{sec:robustness_noisy_dictionary_more}), and provide more examples of language sources used for training (Sec.~\ref{sec:examples_of_language_sources}). Lastly, we explore a cross-frame attention temporal module in Sec.~\ref{sec:parameter_free_temp_module}. 

\section{Source Code}\label{sec:source_code}
We provide the source code in the directory \verb$supplementary_3246/source_code/MAXI$. Check \verb$README.md$ for instructions of re-evaluation. The source code will be released upon acceptance. 

\input{fig/supp_attn_in_dict_samples}

\section{Dataset Statistics}\label{sec:dataset_statistics}
\textbf{Kinetics-400} (K400)~\cite{kay2017kinetics}  is the most popular benchmark for action recognition tasks, containing around 240K training videos in 400 classes. The dataset consists of YouTube videos with an average length of 10 seconds. We use the training set of K400 for finetuning CLIP. 

\textbf{UCF101}~\cite{soomro2012ucf101} is collected from YouTube videos, consisting of 13K videos from 101 classes. There are three splits of training data ($\sim$ 9.4K) and validation data ($\sim$3.6K). Following XLCIP~\cite{ni2022expanding} and ViFi-CLIP~\cite{rasheed2022fine}, we report the average performance on the three validation splits. 

\textbf{HMDB51}~\cite{kuehne2011hmdb} consists of 7K videos comprised of 51 action classes, collected from YouTube videos and movie clips. There are three splits of training data ($\sim$ 3.5K, 70 videos per class) and validation data ($\sim$1.5K, 30 videos per class). Following~\cite{ni2022expanding,rasheed2022fine}, we report the average performance on the three validation splits. 

\textbf{Kinetics-600} (K600)~\cite{carreira2018short} is an extension of K400, consisting of 650K videos in 600 classes. Following~\cite{chen2021elaborative, ni2022expanding, rasheed2022fine}, we use the 220 classes\footnote{In the evolution from K400 to K600, there are renamed, removed and split classes. See details in Appendix B in~\cite{chen2021elaborative}.} that are not included in K400 for zero-shot action recognition. There are three validation splits, each containing 160 classes randomly sampled from these 220 classes. We report the average performance on the three validation splits, each containing around 14K videos. 

\textbf{MiniSSv2}~\cite{chen2021deep} (87 classes, 93K videos) is a subset of Something-Something v2 (SSv2)~\cite{goyal2017something} (174 classes, 220K videos). SSv2 is an egocentric motion-based action dataset, which has a large visual domain shift to K400. Furthermore, the action classes are detailed descriptions of fine-grained movements, in a largely different language style than the K400 action dictionary, \eg \textit{Failing to put something into something because something does not fit}, and \textit{Lifting a surface with something on it but not enough for it to slide down}. For zero-shot action recognition, we evaluate on the validation split of MiniSSv2 (12K videos). For few-shot action recognition, we follow~\cite{rasheed2022fine} and evaluate on the validation split of SSv2 (25K videos).  


\textbf{Charades}~\cite{sigurdsson2016hollywood} is a long-range activity dataset recorded by people in their homes based on provided scripts for home activities. There are $\sim$10K videos in 157 classes. The average video length is 30 seconds. Each video has annotations of an average of 6.8 action instances, often in complex co-occurring cases. The validation split consists of 1.8K videos. We report the mean Average Precision (mAP) for the multi-label classification task. 

\textbf{Moments-in-Time} (MiT)~\cite{monfort2019moments} is a large-scale action dataset of 3-second YouTube video clips, which cover actions in 305 classes, performed by both humans and animals. The validation split consists of 30K videos. 

\textbf{UAV Human} (UAV)~\cite{li2021uav} is an action dataset recorded with an Unmanned Aerial Vehicle in unique camera viewpoints. There are 155 action classes. Actions in different categories are performed by a fixed group of subjects in the same background scenes. This leads to an extremely low object-scene bias and a large shift to the domain of K400 and CLIP. We evaluate on the RGB videos and report the average performance on the two official validation splits, each consisting of $\sim$ 6.2K videos. 

% \wei{explain the issue with UCF class name, with space} we add space to have human-readable class names on UCF101.



\section{Implementation Details}\label{sec:implementation_detials}
In addition to the details mentioned in the main manuscript, we cover more implementation specifics here. 

\textbf{CLIP matching.} 
The CLIP matching step is for consuming the language source of the predefined action dictionary $D$. 
We use CLIP\footnote{CLIP model \href{https://openaipublic.azureedge.net/clip/models/5806e77cd80f8b59890b7e101eabd078d9fb84e6937f9e85e4ecb61988df416f/ViT-B-16.pt}{source} }~\cite{clip} with the ViT-B/16 visual encoder~\cite{dosovitskiy2021image} to match each video with texts in the predefined action dictionary. To improve the matching quality for Text Bag Construction, we perform prompt ensembling over the 28 prompt templates\footnote{\url{https://github.com/openai/CLIP/blob/main/data/prompts.md}} which are proposed by CLIP for Kinetics videos. Important to note, during inference we follow the exact protocol of ViFi-CLIP \cite{rasheed2022fine} and use only a single prompt.
% . 

\textbf{GPT-3 text expansion.}
We employ the GPT-3 \texttt{text-davinci-003} model~\cite{brown2020language}. We set the temperature to 0.4. We generate 5 verb phrases using the input instruction - \textit{Generate 5 phrases to describe the action of $<$action$>$ in simple words}. Here for a video $x_i$, \textit{$<$action$>$} is the best matched text $\hat t_i$ from the predefined action dictionary. 

\textbf{BLIP captioning.}
We use BLIP model \footnote{BLIP model \href{https://storage.googleapis.com/sfr-vision-language-research/BLIP/models/model_large_caption.pth}{source} }~\cite{blip} with ViT-L/16 as the image captioner. For each video, the image captioning is performed on 8 uniformly sampled frames. The frames are resized into 384.

\textbf{Text augmentation}. We use the natural language processing tool spaCy\footnote{spaCy \url{https://spacy.io/}} to parse the verbs and verb phrases from the descriptions. We perform augmentation by converting the verbs into forms of lemma and gerund (present participle) and include results in the text bag. 

\textbf{Training.} We employ CLIP with the ViT-B/16 visual encoder. We follow the full-finetuning configuration of~\cite{rasheed2022fine} to finetune both the visual and text encoder. 
During training, we follow the configuration of~\cite{rasheed2022fine,ni2022expanding} for visual augmentation of multi scale crop, random flipping, color jitering and gray scaling. We do not perform augmentations of MixUp or CutMix. 

As different videos have varying numbers of texts in their bags, we randomly sample $N_{\text{bag}}$ texts from the originally constructed bag in each training iteration. 
For multiple instance learning, we use all the $N_{\text{bag}}$ words in a text bag to form $N_{\text{bag}}$ text prompts for each video. 
The text prompt is in the format of \textit{$<$text1$>$ + $<$text2$>$}.
The first part \textit{$<$text1$>$} is uniform for all the $N_{\text{bag}}$ text prompts. Specifically, we use a hand-crafted prompt template \textit{a photo of $<$action$>$}, where \textit{$<$action$>$} is the best-matched text $\hat t_i$ from the predefined action dictionary (see Eq.~1 in the main manuscript). \textit{$<$text2$>$} is an individual text from the text bag. 
To avoid duplication, we do not use $\hat t_i$ as \textit{$<$text2$>$}.
% For \textit{$<$text2$>$}, we do not consider $\hat t_i$ in the text bag to avoid duplication. 

\textbf{Inference.} We follow~\cite{ni2022expanding,rasheed2022fine} and sample a single view via sparse temporal sampling and spatial center crop. The same single prompt template is used in inference. 

% Train on 4$\times$ A6000

\section{Additional Results}


\input{fig/supp_attn_out_of_dict_samples}
\input{fig/supp_attn_general_action_samples}

\subsection{Attention Heatmaps}\label{sec:attention-heatmaps}
To gain more insights into the performance improvement of \OurMethod, we compare the visualizations of attention heatmaps across several approaches in Fig.~\ref{fig:supp_attn_in_dict_samples}, Fig.~\ref{fig:supp_attn_out_of_dict_samples} and Fig.~\ref{fig:supp_attn_general_action_samples}. \textit{CLIP} is the original CLIP~\cite{clip} without any finetuning. \textit{ViFi-CLIP}~\cite{rasheed2022fine} finetunes CLIP via supervised classification on K400 with ground truth annotations. \textit{\OurMethod} is our approach of unsupervised finetuning with language knowledge. 

We obtain the attention maps by computing the cosine similarity between the patch token features from the visual encoder and the text feature from the text encoder. We visualize the attention maps in several action classes from the downstream datasets used for the zero-shot action recognition task. Based on the relationship between the zero-shot action class and the K400 action dictionary used for training, we categorize the visualizations into 3 groups: (1) In-dictionary action classes which have a verb form (lemma or gerund) directly included in the K400 action dictionary, \eg \textit{clap} and \textit{kick ball} in Fig.~\ref{fig:supp_attn_in_dict_samples}; (2) Novel actions classes which do not have any verb form included in the K400 action dictionary, \eg \textit{wave} and \textit{chew} in Fig.~\ref{fig:supp_attn_out_of_dict_samples}; (3) General actions whose verb form is a basic component of several actions in the K400 action dictionary, \eg \textit{catch}, \textit{hit}, \textit{jump} and \textit{run} in Fig.~\ref{fig:supp_attn_general_action_samples}.

\myparagraph{In-dictionary action classes.} In Fig.~\ref{fig:supp_attn_in_dict_samples}, we visualize two samples of the action \textit{clap} and \textit{kick ball}. \textit{clap} has the same lemma as \textit{clapping} in the K400 dictionary, while \textit{kick ball} has related actions of \textit{kicking field goal} and \textit{kicking soccer ball} in the K400 dictionary. We see that CLIP has incorrectly high attention on object (Fig.~\ref{fig:supp_attn_in_dict_samples}(a), 2nd row) or background scene (Fig.~\ref{fig:supp_attn_in_dict_samples}(b), 2nd row). ViFi-CLIP has cluttered high attention on both the subjects and the background scenes. On the contrary, \OurMethod has more focused attention on the hands (for \textit{clap}) and legs (for \textit{kick ball}). 

In our GPT-3 text bag of \textit{clapping}, related words such as \textit{clap}, \textit{smacking hands}, \textit{slapping palms} and \textit{clapping hands} are included. This strengthens the association between the action \textit{clap} and the body part of hands, and leads to more accurate attention. Furthermore, in BLIP caption verb text bags, the verb \textit{clap} appears several times in frame captions of K400 videos of \textit{clapping}, \textit{giving or receiving award} and \textit{applauding}. This further improves the understanding of \textit{clap}. Similarly, in BLIP frame captions, \textit{kick} is an even more basic verb with large amount of occurrences.

\myparagraph{Novel action classes.} In Fig.~\ref{fig:supp_attn_out_of_dict_samples}, we compare the attention maps for the novel verbs \textit{wave} and \textit{chew} that do not appear in the K400 action dictionary. We see that for \textit{wave}, CLIP and ViFi-CLIP have attention on the background scene or on the head, while \OurMethod has correct attention on the hand and arm. For \textit{chew}, CLIP has more attention on the hair and ViFi-CLIP has attention on a large area of the face. On the contrary, \OurMethod has consistent focused attentions on the area of the mouth where the action  \textit{chew} happens. 

The verb \textit{wave} appears in BLIP caption verb text bags of several K400 videos of \textit{clapping}, \textit{applauding}, \textit{celebrating}. The verb \textit{chew} appears in captions of K400 videos of \textit{eating carrots}, \textit{eating spaghetti}, \textit{eating watermelon} and \textit{baby waking up}. The additional language source improves the knowledge of actions that never appear in the K400 action dictionary. 

\myparagraph{General actions.} In Fig.~\ref{fig:supp_attn_general_action_samples}, we illustrate the attention maps for four general verbs \textit{catch}, \textit{hit}, \textit{jump} and \textit{run}. These verbs are basic components of several actions in the K400 dictionary, \eg \textit{catching fish}, \textit{catching or throwing frisbee}, \textit{hitting baseball}, \textit{jumping into pool} and \textit{running on treadmill}. In these samples, CLIP and ViFi-CLIP have cluttered attention on the background scene or objects. \OurMethod has more concentrated attention on the part where the action happens, \eg catching ball with hands (Fig.~\ref{fig:supp_attn_general_action_samples}(a), last row), hitting drum with stick (Fig.~\ref{fig:supp_attn_general_action_samples}(b), last row), legs and feet jump on stairs (Fig.~\ref{fig:supp_attn_general_action_samples}(c), last row), and attention on the running body (Fig.~\ref{fig:supp_attn_general_action_samples}(d), last row).

These verbs are very general and could have highly diverse instantiations. \Eg \textit{hit} (drum) in Fig.~\ref{fig:supp_attn_general_action_samples}(b) is not close to \textit{hitting baseball} on K400. \textit{jump} (on stairs) in Fig.~\ref{fig:supp_attn_general_action_samples}(c) is not close to \textit{jumping into pool} or \textit{bungee jumping} on K400, even if they share the same verb. In our GPT-3 verb bag and BLIP caption verb bag, there is a large amount of these verb instances that facilitate the comprehensive understanding of these general verbs. This leads to better focus even in unusual complex scenes, \eg jumping on stairs (Fig.~\ref{fig:supp_attn_general_action_samples}(c)). 




% CLIP has object bias and tends to have attention on the distinct objects. 

\input{tab/supp_noisy_class_space}
\input{fig/caption_gpt_examples}
\input{tab/supp_temp_att}
\subsection{Robustness Against Noisy Action Dictionary}\label{sec:robustness_noisy_dictionary_more}
In Table~5 in the main manuscript, we explored the robustness of our finetuning pipeline against noisy action dictionaries. In case of an over-specified dictionary, we added noisy verbs and verb phrases into the original K400 action dictionary. The noisy verbs are parsed from the captions in the WebVid2.5M dataset~\cite{bain2021frozen}. Here we further increase the ratio of noisy verbs, and add 800 and 1200 verbs into the dictionary, resulting in 1200-class and 1600-class spaces. 

In Table~\ref{tab:supp_noisy_class_space}, we report the zero-shot transfer performance of models finetuned with the resulted 1200-class and 1600-class space. We set the text bag filtering ratio $p=50\%$ for improved text bag quality. We see that even with extremely noisy dictionary where 50\% to 75\% of words do not match with the video data, our finetuning still results in a robust zero-shot transfer performance to unseen datasets. 
The robustness is the consequence of the fact that we collect knowledge from multiple language sources and learn from them via Multiple Instance Learning.
Note that the zero-shot transfer does not have consistent change in performance across the downstream datasets, as different datasets have different language domain shift to the action dictionary used for training. 



\subsection{Examples of Language Sources}\label{sec:examples_of_language_sources}
Similar to the \textit{cooking egg} example in Fig.~2 in the main manuscript, we illustrate more examples of video frames, BLIP frame captions, GPT-3 phrases, together with the derived BLIP verb bag and GPT-3 verb bag in Fig.~\ref{fig:caption_gpt_examples}. The videos are from the unlabeled K400 dataset which we use for training. 



\subsection{Parameter-Free Temporal Module}\label{sec:parameter_free_temp_module}
As mentioned in Sec.~3.1 in the main manuscript, we explore a parameter-free temporal-aware module on the CLIP model. We modify the multi head attention module~\cite{vaswani2017attention} in the visual encoder of CLIP to be temporal aware. Originally, the attention on the frame $t$ is computed via 
$A_t(Q_t, K_t, V_t)= \text{softmax}\frac{Q_t {K_t}^\top }{d_k}V_t$, where $Q_t$, $K_t$ and $V_t$ are the query, key and value from frame $t$. 

We explore to compute the cross-frame attention via 
\begin{equation}
\small
A'_t(Q_t, K_{t+i}|_{i\in I}, V_t)= 
\text{softmax}
\frac{ \sum_{i\in I} (Q_t \cdot {K_{t+i}}^\top) / |I|}
{d_k}V_t
\end{equation}
where we set $I=\{-1, 0, 1\}$. In this case, we use the keys from the frame $t-1$, $t$ and $t+1$ to compute the attention for frame $t$. 

We apply the cross-frame attention on the last 2 and on the last 6 transformer layers in the visual encoder of CLIP. In Table~\ref{tab:supp_tempt_att}, we report the zero-shot transfer performance. We see that in comparison to the variant without any temporal attention module, using cross-frame attention does not lead to performance improvement. K400 is of far smaller scale in comparison to the original CLIP domain. Finetuning from the CLIP model weights with a modified architecture could result in the case that the model drifts far away from the wise CLIP source domain. The results are consistent with the claims in \cite{rasheed2022fine} that a sophisticated temporal module does not necessarily lead to performance improvement.
% (2) K400 contains YouTube videos where the temporal reasoning does not have a big impact on recognizing actions. 




% \textbf{We do not add additional parameters onto CLIP}. 

% Explanation: K400 is of a lot smaller scale in comparison to the original CLIP source domain. as we finetune the entire model, optimization is sensitive, the model could easily drift away. on online user videos, the temporal reasoning does not have a big impact. 

